Neural Machine Translation of Text from Non-Native Speakers

Neural Machine Translation (NMT) systems are known to degrade when confronted with noisy data, especially when the system is trained only on clean data. In this paper, we show that augmenting training data with sentences containing artificially-introduced grammatical errors can make the system more robust to such errors. In combination with an automatic grammar error correction system, we can recover 1.5 BLEU out of 2.4 BLEU lost due to grammatical errors. We also present a set of Spanish translations of the JFLEG grammar error correction corpus, which allows for testing NMT robustness to real grammatical errors.

==> article_anal.tex <==

\begin{table}[t]
    \centering
    \begin{tabular}{c|ccccc}
    \toprule
        %\multicolumn{6}{c}{BLEU $\Delta$: WMT-\art{} - WMT-\textsc{clean}}\\
        Correct & \multicolumn{5}{c}{Substituted article}  \\
         article & a & an & the & {\emp} & \multicolumn{1}{c}{\emph{all}} \\
    \midrule
        a & -- & 0 & $-1.4$ & $-2.2$ & $-2.0$ \\
        an & 0 & -- & $-4.0$ & $-1.3$ & $-0.7$  \\
        the & $-1.8$ & $-0.7$ & -- & $-1.3$ & $-1.3$ \\
        {\emp} & $-1.3$ & $-0.2$ & $-0.4$  & -- & $-0.5$ \\
        \emph{all} & $-1.4$ & $-0.4$ & $-0.4$ & $-1.3$ & $-0.8$ \\
    \bottomrule
    \end{tabular}
    \caption{Effect of article substitutions in test data (\art{}) relative to clean test data (\clean{}), broken down by substitution type. Different article substitutions have very different impacts on BLEU; changing an indefinite article to definite is especially damaging.}
    \label{tab:art}
\end{table}


==> prep_anal.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{cc}
    \toprule
        Substitution & BLEU difference \\ %$\Delta$ \\
        %& WMT-\prep{} - WMT-\textsc{clean} \\
    \midrule
        in$\rightarrow$by & $-3.4$ \\
        on$\rightarrow$to & $-3.2$ \\
        for$\rightarrow$on & $-2.9$ \\
        in$\rightarrow$from & $-2.7$ \\
        in$\rightarrow$of & $-2.4$ \\
    \midrule
        {\emp}$\rightarrow$\emph{any} & $-0.5$ \\
        \emph{any}$\rightarrow${\emp} & $-2.0$ \\
    \bottomrule
    \end{tabular}
    \caption{Effect of selected preposition substitutions in test data (WMT-\prep) relative to clean test data (WMT-\clean). Deleting a correct preposition leads to much worse performance that inserting an incorrect preposition.}
    \label{tab:prep}
\end{table}

==> robustness.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|cc|cc|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Training} &  \multicolumn{10}{c}{a) WMT Test Set}\\
          & \drop & $\Delta$ & \art & $\Delta$  & \prep & $\Delta$  & \nn & $\Delta$  &\sva & $\Delta$  \\
        \midrule
        \clean & 75.1 & \xt{+1.9}& 80.3 &\xt{+0.9} & 83.7 &\xt{+0.3} & 75.1 & \xt{+3.3} & 87.2 &\xt{-0.1} \\
        \mixd & 77.0 && 81.2 && 84.0 && 78.4 && 87.1 \\
        \midrule\midrule
        & \multicolumn{10}{c}{ b) \jfleges Dev Set} \\
        & \textsc{cor0} & $\Delta$ & \textsc{cor1} & $\Delta$  & \textsc{cor2} & $\Delta$  & \textsc{cor3} & $\Delta$  & \textsc{all-cor} & $\Delta$  \\
        \cmidrule{2-11}
        \clean & 55.2 & \xt{+0}
        & 53.5 & \xt{+0.8} & 59.8 & \xt{+0.5} & 62.4 & \xt{+1.8} & 78.1 & \xt{+1.4} \\
        \mixd & 55.2 && 54.2 && 60.3 && 64.2 && 79.5 & \\
        \midrule
        & \multicolumn{10}{c}{c) \jfleges Test Set} \\
        & \textsc{cor0} & $\Delta$  & \textsc{cor1} & $\Delta$  & \textsc{cor2} & $\Delta$  & \textsc{cor3} & $\Delta$  & \textsc{all-cor} & $\Delta$  \\
        \cmidrule{2-11}
        \clean & 59.7 & \xt{+2.8} & 61.3 & \xt{+2.8} & 57.9 & \xt{+2.2} & 52.9 & \xt{+3.1} & 74.9 & \xt{+2.8}\\
        \mixd  & 62.9 && 64.1 && 60.1 && 56.0 && 77.7 & \\
    \bottomrule
    \end{tabular}
    \caption{\emph{a)}: Robustness on each type of error, computed with BLEU against the produced translation of the clean sentence. We find that our proposed solution (\textsc{mix-both}) is generally more robust.\\
    \emph{b,c)}: Robustness against \jfleg correction sets. For \jfleges \textsc{all-cor} we use multi-reference BLEU against the translations of all four \jfleges references. Again, \mixd outperforms the \clean model.}
    \label{tab:robust1}
\end{table*}
